Sensitivity Analysis for Vehicle Dynamics Models -- An Approach to Model Quality Assessment for Automated Vehicles

Model-based approaches have become increasingly popular in the domain of automated driving. This includes runtime algorithms, such as Model Predictive Control, as well as formal and simulative approaches for the verification of automated vehicle functions. With this trend, the quality of models becomes crucial for automated vehicle safety. Established tools from model theory which can be applied to assure model quality are uncertainty and sensitivity analysis [1]. In this paper, we conduct sensitivity analyses for a single and double track vehicle dynamics model to gain insights about the models' behavior under different operating conditions. We compare the models, point out the most important findings regarding the obtained parameters sensitivities, and provide examples of possible applications of the gained insights.

==> shapes.tex <==
%
%
\makeatletter

\pgfdeclareshape{openinterface}
{
  \inheritsavedanchors[from=circle] %
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
}
\pgfdeclareshape{interface}
{
  \inheritsavedanchors[from=circle] %
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{.95\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
  \foregroundpath{
	 \centerpoint
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
    \pgfutil@tempdimb=\radius%
	 \advance\pgfutil@tempdima by-.25\pgfutil@tempdima%
	 \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+.25\pgfutil@tempdimb}{0pt}}}{\pgfutil@tempdima}
	 \pgfusepath{fill}
  }
}
%
\pgfdeclareshape{umlcomponent}
{
  \inheritsavedanchors[from=rectangle] %
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \backgroundpath{
	  \newdimen\pgf@xd\newdimen\pgf@yd
	  \newdimen\pgf@xe\newdimen\pgf@ye
	  \newdimen\pgf@xf\newdimen\pgf@yf
		%
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		%
		\pgf@xc=\pgf@xa \pgf@yc=.5\pgf@yb \advance\pgf@yc by .5\pgf@ya
		\pgf@yd=.3\pgf@yb
		\pgf@ye=.2\pgf@yb
%
%
%
		%
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathclose
		%
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
  }
}

%
\pgfarrowsdeclare{srvarrow}{srvarrow}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.4\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.5\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{white}
  \pgfusepathqfill
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.8\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke
  \pgftransformshift{\pgfqpoint{-0.5\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.55\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill
}

\pgfarrowsdeclare{srvrequired}{srvrequired}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{1.3\pgfutil@tempdima}{0.95\pgfutil@tempdima}}}%
  \pgfpatharc{80}{280}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke 
}

\pgfarrowsdeclare{srvprovided}{srvprovided}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.4\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill 
}
\makeatother

